Measuring LDA Topic Stability from Clusters of Replicated Runs

Background: Unstructured and textual data is increasing rapidly and Latent Dirichlet Allocation (LDA) topic modeling is a popular data analysis methods for it. Past work suggests that instability of LDA topics may lead to systematic errors. Aim: We propose a method that relies on replicated LDA runs, clustering, and providing a stability metric for the topics. Method: We generate k LDA topics and replicate this process n times resulting in n*k topics. Then we use K-medioids to cluster the n*k topics to k clusters. The k clusters now represent the original LDA topics and we present them like normal LDA topics showing the ten most probable words. For the clusters, we try multiple stability metrics, out of which we recommend Rank-Biased Overlap, showing the stability of the topics inside the clusters. Results: We provide an initial validation where our method is used for 270,000 Mozilla Firefox commit messages with k=20 and n=20. We show how our topic stability metrics are related to the contents of the topics. Conclusions: Advances in text mining enable us to analyze large masses of text in software engineering but non-deterministic algorithms, such as LDA, may lead to unreplicable conclusions. Our approach makes LDA stability transparent and is also complementary rather than alternative to many prior works that focus on LDA parameter tuning.

==> 4_results_more_hide_in_the_end.tex <==

\begin{table*}
\caption {Weekend topics k=20 rbo p 0.95} \label{tab:weekend20} 
% latex table generated in R 3.4.2 by xtable 1.8-2 package
% Mon Jun 25 13:42:32 2018
\begin{tabular}{rllllllllll}
  \hline
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\ 
  \hline
Silhouette & 0.954 & 0.985 & 0.862 & 0.816 & 0.629 & 0.630 & 0.632 & 0.426 & 0.618 & 0.310 \\ 
  Spearman & 0.953 & 0.907 & 0.716 & 0.783 & 0.385 & 0.348 & 0.403 & 0.255 & 0.255 & 0.389 \\ 
  Jaccard & 0.813 & 0.759 & 0.767 & 0.708 & 0.493 & 0.550 & 0.562 & 0.506 & 0.462 & 0.448 \\ 
  RBO & 0.926 & 0.878 & 0.851 & 0.841 & 0.682 & 0.668 & 0.646 & 0.633 & 0.607 & 0.595 \\ 
  Topics & 20 & 20 & 20 & 20 & 17 & 24 & 23 & 17 & 22 & 11 \\ 
  1 & backed & id & tab & test & fix & patch & media & js & build & check \\ 
  2 & changeset & commit & button & tests & bustage & change & data & add & files & null \\ 
  3 & tree & mozreview & menu & fix & build & need & audio & src & use & fix \\ 
  4 & closed & add & search & disable & followup & used & video & fix & builds & error \\ 
  5 & backout & remove & ui & add & port & changes & time & jit & file & return \\ 
  6 & bustage & update & panel & intermittent & patch & makes & use & ionmonkey & support & crash \\ 
  7 & failures & stylo & window & enable & error & animation & add & nbp & add & value \\ 
  8 & changesets & test & tabs & html & follow & case & stream & use & update & add \\ 
  9 & build & rename & windows & failures & rs & time & track & implement & version & assertion \\ 
  10 & mochitest & use & page & mochitest & warning & set & buffer & rename & windows & handle \\ 
   \hline
\end{tabular}
\end{table*}


\begin{table*}
\caption {Weekend topics k=20 rbo p 0.95} \label{tab:weekend20} 
% Sun Jun 24 13:28:34 2018
% latex table generated in R 3.4.2 by xtable 1.8-2 package
% Mon Jun 25 13:42:33 2018
\begin{tabular}{rllllllllll}
  \hline
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\ 
  \hline
Silhouette & 0.409 & 0.599 & 0.366 & 0.413 & 0.453 & 0.341 & 0.452 & 0.108 & 0.187 & 0.092 \\ 
  Spearman &  0.197 &  0.145 &  0.132 &  0.037 & -0.031 & -0.139 & -0.108 & -0.172 & -0.220 & -0.295 \\ 
  Jaccard & 0.395 & 0.362 & 0.408 & 0.340 & 0.395 & 0.298 & 0.330 & 0.299 & 0.268 & 0.289 \\ 
  RBO & 0.580 & 0.568 & 0.550 & 0.496 & 0.487 & 0.437 & 0.420 & 0.393 & 0.374 & 0.374 \\ 
  Topics & 20 & 19 & 19 & 20 & 21 & 21 & 29 & 14 & 25 & 18 \\ 
  1 & use & remove & add & thread & cache & event & frame & add & add & update \\ 
  2 & instead & unused & default & main & content & events & use & tests & use & add \\ 
  3 & return & unnecessary & pref & shutdown & add & content & image & test & object & https \\ 
  4 & type & fix & support & process & use & element & size & dom & objects & style \\ 
  5 & value & rename & enable & event & sicking & input & layer & use & implement & servo \\ 
  6 & add & clean & use & avoid & data & window & scroll & browser & dom & changes \\ 
  7 & string & variable & windows & crash & http & selection & text & devtools & js & source \\ 
  8 & class & replace & disable & ensure & api & key & css & js & function & patch \\ 
  9 & function & longer & plugin & message & service & document & display & remove & functions & css \\ 
  10 & convert & function & e10s & use & load & text & layers & api & class & support \\ 
   \hline
\end{tabular}
\end{table*}




\begin{table*}
\caption {Weekend topics k=20 rbo p 0.9} \label{tab:weekend20} 
% latex table generated in R 3.4.2 by xtable 1.8-2 package
% Mon Jun 25 13:42:32 2018
% Mon Jun 25 16:18:44 2018
\begin{tabular}{rllllllllll}
  \hline
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\ 
  \hline
Silhouette & 0.954 & 0.985 & 0.816 & 0.862 & 0.629 & 0.630 & 0.426 & 0.599 & 0.632 & 0.409 \\ 
  Spearman & 0.953 & 0.907 & 0.783 & 0.716 & 0.385 & 0.348 & 0.255 & 0.145 & 0.403 & 0.197 \\ 
  Jaccard & 0.813 & 0.759 & 0.708 & 0.767 & 0.493 & 0.550 & 0.506 & 0.362 & 0.562 & 0.395 \\ 
  RBO & 0.948 & 0.888 & 0.861 & 0.845 & 0.705 & 0.671 & 0.624 & 0.615 & 0.615 & 0.615 \\ 
  Topics & 20 & 20 & 20 & 20 & 17 & 24 & 17 & 19 & 23 & 20 \\ 
  1 & backed & id & test & tab & fix & patch & js & remove & media & use \\ 
  2 & changeset & commit & tests & button & bustage & change & add & unused & data & instead \\ 
  3 & tree & mozreview & fix & menu & build & need & src & unnecessary & audio & return \\ 
  4 & closed & add & disable & search & followup & used & fix & fix & video & type \\ 
  5 & backout & remove & add & ui & port & changes & jit & rename & time & value \\ 
  6 & bustage & update & intermittent & panel & patch & makes & ionmonkey & clean & use & add \\ 
  7 & failures & stylo & enable & window & error & animation & nbp & variable & add & string \\ 
  8 & changesets & test & html & tabs & follow & case & use & replace & stream & class \\ 
  9 & build & rename & failures & windows & rs & time & implement & longer & track & function \\ 
  10 & mochitest & use & mochitest & page & warning & set & rename & function & buffer & convert \\ 
   \hline
\end{tabular}
\end{table*}


\begin{table*}
\caption {Weekend topics k=20 p 0.9} \label{tab:weekend20} 
% Sun Jun 24 13:28:34 2018
% latex table generated in R 3.4.2 by xtable 1.8-2 package
% Mon Jun 25 13:42:33 2018
% Mon Jun 25 16:18:44 2018
\begin{tabular}{rllllllllll}
  \hline
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\ 
  \hline
Silhouette & 0.618 & 0.310 & 0.366 & 0.413 & 0.453 & 0.341 & 0.452 & 0.187 & 0.108 & 0.092 \\ 
  Spearman &  0.255 &  0.389 &  0.132 &  0.037 & -0.031 & -0.139 & -0.108 & -0.220 & -0.172 & -0.295 \\ 
  Jaccard & 0.462 & 0.448 & 0.408 & 0.340 & 0.395 & 0.298 & 0.330 & 0.268 & 0.299 & 0.289 \\ 
  RBO & 0.605 & 0.579 & 0.549 & 0.503 & 0.450 & 0.449 & 0.401 & 0.360 & 0.350 & 0.335 \\ 
  Topics & 22 & 11 & 19 & 20 & 21 & 21 & 29 & 25 & 14 & 18 \\ 
  1 & build & check & add & thread & cache & event & frame & add & add & update \\ 
  2 & files & null & default & main & content & events & use & use & tests & add \\ 
  3 & use & fix & pref & shutdown & add & content & image & object & test & https \\ 
  4 & builds & error & support & process & use & element & size & objects & dom & style \\ 
  5 & file & return & enable & event & sicking & input & layer & implement & use & servo \\ 
  6 & support & crash & use & avoid & data & window & scroll & dom & browser & changes \\ 
  7 & add & value & windows & crash & http & selection & text & js & devtools & source \\ 
  8 & update & add & disable & ensure & api & key & css & function & js & patch \\ 
  9 & version & assertion & plugin & message & service & document & display & functions & remove & css \\ 
  10 & windows & handle & e10s & use & load & text & layers & class & api & support \\ 
   \hline
\end{tabular}
\end{table*}

==> 98_attic.tex <==


LDA involves multiple input parameters that effect the outcome of the topic model and it recognized that the best setting of these input parameters varies between data sets \cite{agrawal2016wrong, binkley2014understanding,panichella2013effectively}. 



\section{Results}
Here we demonstrate our method. We are fully awere that this demonstration can only illustrate our method and further empirical studies are required to understand 



\subsection{Preprocessing}
We aimed for minimal preprocessing to make sure our method we applicable to different context. Lower caseing remove numbers. Used R tokenizers packages

However, for Firefox commits we needed to remove names that are used to indicate who should review the contribution but have nothing to do with the content of the commit itself. Also the letter codes used for various actions a (approval), r(review) and sr(super) review were reveied



\subsection{Optimizing parameters}
Our training target was perplexity as it is commonly used target for LDA modeling. We first used differential evolution to find optimal values for number of topics (k) and hyper parameters alpha and beta. However, we found that the number of topics started to become very large, e.g. number of input documents divided by five, while beta approaches to zero. We found a  research presentation showing similar graphs suggesting this might be a more genenral issues. REF Slide 13
%http://phusewiki.org/wiki/images/c/c9/Weizhong_Presentation_CDER_Nov_9th.pdf
Clustering for example 50,000 documents to 10,000 topics makes very little sense so we settled for fixed sizes of k 20, 100, and 500 while still using differential evolution to train for best hyper parameters alpha and beta. We then used these values to train our LDA models. 


\subsection{LDA instability}
Prior works have addressed LDA instability by using a Jacard similarity derivate as training target to find optimal number of topics and values for hyper parameters alpha and beta. mension paper lda ge paperi. We recognize that LDA instability is a problem that might lead in to making wrong conclusions. 
To overcome LDA instability in this paper we  train multiple LDA models and cluster them later to present researcher a compact view of the found topics. We also provide cohenrence measure of each cluster allowing humans to interpert cluster coherence. Additionally, our method enables exploration of all of the individual topics of for each cluster for more detailed investigation. Additional, concequence of our method is that parameter optimizations (k, alpha and beta), can have other training targets than similarity measures, ones that are typically used are log-likelihood ref, perplexity and currently 



\subsection{Enhancing LDA topic relevance}
LDA often proposes too general words for a topic when a humans would prefer to see words that are less general and more topic specific. To address this problem researchers have suggested using word relevance score to order words for a topic \cite{sievert2014ldavis}. Relevance was defined as follows. 
$$ relevance = \lambda log(\theta_{kw}) + (1 - \lambda) log (\theta_{kw} / p_w) $$

In the equaltaion \textlambda{ } is between 0 and 1. When \textlambda{ } is 1 it means that only original word probabilities  \straighttheta{ } for topics are used. When \textlambda{ } is 0 it means that only the latter part of the equation is used where the original word probabilities  \straighttheta{ } are dividived p\textsubscript{w}  marginal probabilities of each term. This provides lift to rare words as their marginal probabilities are lower and marginal probability is used to divide the orignal LDA word probabbilties. In the equation \textit{k} denotes a topic while \textit{w} denotes a term. Through an empirical investigation \cite{sievert2014ldavis} finds \textlambda = 0.6 as the optimal which we also use in this work. For all topic-word matrix computations that follow we use the relevances instead of orginal topic-word probabilties provided by the LDA clustering. 


\subsection{Measuring group differences}
In order to present differences between documents we obviously need to know the group each document belongs. The groups can be anything day vs night or before and after particular software process change. In LDA each document consists of probabilities of all topics expressed as theta. Similar to Giffins and Saewers we sum up these probabilties for both groups and this way we can compute how probable each document is in both groups (WHAT about unqual group sizes)  



\subsection{Clustering and compressing produced LDA topics}
Due to LDA instability we do several runs of LDA and each might give slightly result of the group difference. For example if we do 10 LDA runs and pick 10 most probable topics for particular group we end up with 100 topics describing that group. For human reader it is   highly helpful to cluster the topics. A simple approach would be to simply take the top ten words of each topic form a document (topic) term matrix and compute similarities. A binary coding for each word while but also the word probabilities produced by LDA could also be used. We tried both of these approaches but found the clustering results unsatisfactory as document term counts do consider the similarity of words, e.g. words "unnessary" and "redundant" have similar meaning. We also found that clustering and specially for optimal number of cluster could be slow as number of terms in the document term matrix becomes larger.     For those reasons we decided to convert document term matrix consisting of word probablities produced by LDA to vector space




Hyperparameters reprenet phishopical viewpoints. How many topics does one document really have. 

There is no correct number of topics. Just different targets towards to train for

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI
